GTA: Generative Trajectory Augmentation with Guidance for Offline Reinforcement Learning

Offline Reinforcement Learning (Offline RL) presents challenges of learning effective decision-making policies from static datasets without any online interactions. Data augmentation techniques, such as noise injection and data synthesizing, aim to improve Q-function approximation by smoothing the learned state-action region. However, these methods often fall short of directly improving the quality of offline datasets, leading to suboptimal results. In response, we introduce GTA, Generative Trajectory Augmentation, a novel generative data augmentation approach designed to enrich offline data by augmenting trajectories to be both high-rewarding and dynamically plausible. GTA applies a diffusion model within the data augmentation framework. GTA partially noises original trajectories and then denoises them with classifier-free guidance via conditioning on amplified return value. Our results show that GTA, as a general data augmentation strategy, enhances the performance of widely used offline RL algorithms across various tasks with unique challenges. Furthermore, we conduct a quality analysis of data augmented by GTA and demonstrate that GTA improves the quality of the data. Our code is available at https://github.com/Jaewoopudding/GTA

==> tables/Ablations_isadaptive.tex <==
\begin{table}[t]
% \vspace{-5pt}
\centering
\caption{Ablations on Amplified return conditioning.}
\resizebox{0.5\linewidth}{!}{
\begin{tabular}{c|cccc}
\toprule
\multirow{2}{*}{\makecell{metric}} &\multirow{2}{*}{\makecell{Offline data}}   &\multirow{2}{*}{\makecell{Fixed}} &\multirow{2}{*}{\makecell{Unconditioned}} & \multirow{2}{*}{\makecell{Amplified\\ (ours)}}  \\
\\
\midrule
D4RL score &48.65 \footnotesize{$\pm$ 0.31} & 52.70 \footnotesize{$\pm$ 0.20} & 49.29 \footnotesize{$\pm$ 0.38}& 57.41 \footnotesize{$\pm$ 0.53}\\
Oracle reward &4.77& 6.24  & 4.92 & 6.54  \\
\midrule
\end{tabular}}
\vspace{-12pt}
\label{table:ablation_isadpative}
\end{table}


==> tables/antmaze.tex <==
\begin{table*}
\centering
\caption{
Normalized average scores on complex robotics tasks like D4RL Antmaze tasks, with the highest scores highlighted in \textbf{bold}. Each cell displays the mean and standard deviation from 10 evaluations using 4 seeds. All offline RL algorithms trained with dataset augmented by GTA outperform other data augmentation baselines at average scores.}

\resizebox{\linewidth}{!}{
\begin{tabular}{cc|cccccc|c}
\toprule

\multirow{2}{*}{\makecell{\textbf{Algo.}}} &\multirow{2}{*}{\textbf{Aug.}}

& \multicolumn{6}{c|}{\textbf{Antmaze}} & \multirow{2}{*}{\textbf{Average}} \\

&& umaze & medium-play & large-play & umaze-diverse & medium-diverse & large-diverse & \\

\cmidrule{1-9}

& None & 44.64 \footnotesize{$\pm$ 0.71}  & 89.48 \footnotesize{$\pm$ 5.50}  & 61.04 \footnotesize{$\pm$ 3.18}  & 65.69 \footnotesize{$\pm$ 24.41}  & 104.08 \footnotesize{$\pm$ 5.81}  & 84.58 \footnotesize{$\pm$ 1.92}  & 84.11 \footnotesize{$\pm$ 4.12}    \\

&S4RL & 44.53 \footnotesize{$\pm$ 0.30}  & 90.78 \footnotesize{$\pm$ 4.65}  & 59.34 \footnotesize{$\pm$ 3.50}  & 67.39 \footnotesize{$\pm$ 23.81}  & 106.10 \footnotesize{$\pm$ 7.24}  & 84.63 \footnotesize{$\pm$ 2.44}  & 83.42 \footnotesize{$\pm$ 4.70}   \\

&SynthER & 45.57 \footnotesize{$\pm$ 0.34}  & 85.47 \footnotesize{$\pm$ 11.35}  & \textbf{63.70 \footnotesize{$\pm$ 3.69} } & 78.81 \footnotesize{$\pm$ 15.80}  & 98.99 \footnotesize{$\pm$ 11.27}  & 85.43 \footnotesize{$\pm$ 1.14}  & 90.67 \footnotesize{$\pm$ 1.56}    \\

\rowcolor{Gray}\cellcolor{White}\multirow{-4}{*}{IQL} &GTA  & \textbf{50.04 \footnotesize{$\pm$ 0.84} } & \textbf{93.13 \footnotesize{$\pm$ 3.07} } & 60.89 \footnotesize{$\pm$ 2.91}  & \textbf{89.31 \footnotesize{$\pm$ 16.84} } & \textbf{110.40 \footnotesize{$\pm$ 4.04} } & \textbf{86.69 \footnotesize{$\pm$ 0.89} } & \textbf{93.82 \footnotesize{$\pm$ 1.74} } 
\\



\bottomrule
\end{tabular}}
\vspace{-0pt}
\label{table:antmaze}
\end{table*}



==> tables/batch_size_maze.tex <==
\begin{table}[h]
\centering
\caption{Normalized average scores on D4RL Maze2d tasks}
% \vspace{7pt}
\resizebox{0.45\linewidth}{!}{
\begin{tabular}{cc|ccc|c}
\toprule
\multirow{2}{*}{\makecell{\textbf{Algo.}}} &\multirow{2}{*}{\textbf{Aug.}}

& \multicolumn{3}{c|}{\textbf{Maze2d}} & \multirow{2}{*}{\textbf{Average}} \\

&& umaze & medium & large \\

\cmidrule{1-6}


\multirow{2}{*}{TD3BC} & 256 & 29.41 \footnotesize{$\pm$ 12.31} & 59.45 \footnotesize{$\pm$ 36.25} & 97.10 \footnotesize{$\pm$ 25.41} & 61.99 \footnotesize{$\pm$ 24.65} \\
&\rowcolor{Gray} 1024 & 29.20 \footnotesize{$\pm$ 17.2} & 51.95 \footnotesize{$\pm$ 28.43} & 100.62 \footnotesize{$\pm$ 66.02} & 60.59 \footnotesize{$\pm$ 37.22} \\
\midrule
\multirow{2}{*}{CQL} &256 & -8.90 \footnotesize{$\pm$ 6.11} & 86.11 \footnotesize{$\pm$ 9.68} & 23.75 \footnotesize{$\pm$ 36.70} & 33.65 \footnotesize{$\pm$ 17.50} 
 \\
&\rowcolor{Gray} 1024 &  27.54 \footnotesize{$\pm$ 82.73} & 87.44 \footnotesize{$\pm$ 9.26} & 11.29 \footnotesize{$\pm$ 25.04} & 42.09 \footnotesize{$\pm$ 39.01} \\
\midrule
\multirow{2}{*}{IQL} &256 & 42.11 \footnotesize{$\pm$ 0.58} & 34.85 \footnotesize{$\pm$ 2.72} & 61.72 \footnotesize{$\pm$ 3.50} & 46.23 \footnotesize{$\pm$ 2.27} \\
&\rowcolor{Gray} 1024 & 37.17 \footnotesize{$\pm$ 3.56} & 33.51 \footnotesize{$\pm$ 1.63} & 63.12 \footnotesize{$\pm$ 5.30} & 44.60 \footnotesize{$\pm$ 3.50} \\
\midrule
\multirow{2}{*}{MCQ} &256 & 40.0 \footnotesize{$\pm$ 25.9} & 106.8 \footnotesize{$\pm$ 38.4} & 58.4 \footnotesize{$\pm$ 41.7} & 68.4 \footnotesize{$\pm$ 35.3} \\
&\rowcolor{Gray} 1024 & 44.64 \footnotesize{$\pm$ 3.3} & 111.33 \footnotesize{$\pm$ 34.16} & 56.39 \footnotesize{$\pm$ 31.05} & 70.79 \footnotesize{$\pm$ 22.84} \\




\bottomrule
\end{tabular}}
\vspace{-15pt}
\label{table:batch_size_maze}
\end{table}

==> tables/compare_quality.tex <==
\begin{table}[]
\centering
% \vspace{-5pt}
\caption{Data quality of various augmentation approaches.GTA outperforms other augmentation baselines in terms of optimality, novelty, and diversity while preserving a comparable level of dynamic plausibility.}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{c|cccc}
\toprule
\multirow{1}{*}{\makecell{}}&\multirow{1}{*}{\makecell{Offline Data}}   &\multirow{1}{*}{\makecell{SynthER}} &\multirow{1}{*}{\makecell{S4RL}}& \multirow{1}{*}{\makecell{GTA}}  \\
\midrule
Dynamic MSE ($\downarrow$) ($\times 10^{-2}$)& 0.00  & 0.82 & 0.00 & 0.92\\
Oracle reward ($\uparrow$) & 4.77  & 4.77& 4.77& 6.54 \\
Novelty ($\uparrow$)&-  & 20.40 & 20.50 & 21.24\\

\bottomrule
\end{tabular}}
% }
\vspace{-10pt}
\label{table:compare_quality}
\end{table}


==> tables/hyperparam_reweighting_maze2d.tex <==
\begin{table}[h]
\centering
\caption{Reweighting hyperparameters}
% \resizebox{0.85\linewidth}{!}{
\begin{tabular}{c|clll}
\toprule
Environment & Reweighting & $v_j$ \\
\midrule

Maze2d-umaze-v1 & O & 10  \\
Maze2d-medium-v1 & O & 10\\
Maze2d-large-v1 & O & 5 \\

\bottomrule
\end{tabular}
% }
\label{table:hyperparam_reweighting_maze2d}
\end{table}

==> tables/hyperparameter_mualpha.tex <==
\begin{table}[h]
\centering
\caption{Hyperparameter setting for partial noising level $\mu$ and guidance multiplier $\alpha$}
% \resizebox{0.85\linewidth}{!}{
\begin{tabular}{c|clll}
\toprule
Environment & $\alpha$ & $\mu$ \\
\midrule
Halfcheetah-medium-v2 & 1.3 & 0.5  \\
Halfcheetah-medium-replay-v2 & 1.3 & 0.5  \\
Halfcheetah-medium-expert-v2& 1.3 & 0.25 \\
Hopper-medium-v2& 1.3 & 0.5 \\
Hopper-medium-replay-v2& 1.3 & 0.5\\
Hopper-medium-expert-v2 & 1.3 & 0.5 \\
Walker2d-medium-v2  & 1.1 & 0.5 \\
Walker2d-medium-replay-v2  & 1.3 & 0.5\\
Walker2d-medium-expert-v2  & 1.3 & 0.5\\
maze2d-umaze-v1 &1.1&0.5\\
maze2d-medium-v1 &1.1&0.5\\
maze2d-large-v1 &1.3&0.5\\

\bottomrule
\end{tabular}
% }
\label{table:hyperparam_mualpha}
\end{table}

==> tables/limited_halfcheetah.tex <==


\begin{table}[h]
\centering
\caption{Sensitivity test on partial noising level $\mu$ and guidance multiplier $\alpha$}
% \resizebox{0.9\linewidth}{!}{
\begin{tabular}{c|cccccc}
\toprule
 &  $5\% $ & $10\%$ & $15\%$ & $20\%$ & $100\%$ \\
\midrule
TD3BC &  46.96 \footnotesize{$\pm$ 0.34 } & 48.28 \footnotesize{$\pm$ 0.21 } & 48.36 \footnotesize{$\pm$ 0.25 } & 48.33 \footnotesize{$\pm$ 0.21 } & 48.65 \footnotesize{$\pm$ 0.31 }
\\
TD3BC + GTA & 52.81 \footnotesize{$\pm$ 0.29 } & 53.49 \footnotesize{$\pm$ 0.38 } & 53.63 \footnotesize{$\pm$ 1.92 } & 55.39 \footnotesize{$\pm$ 0.61 } & 57.41 \footnotesize{$\pm$ 0.53 }  

\\
\midrule
\end{tabular}
% }
\label{table:sensitivity_test}
\end{table}
%>{\columncolor{Gray}}

==> tables/mazes.tex <==
\begin{table*}[h!]
\centering
\caption{
Normalized average scores on Maze2d and AntMaze tasks from 10 evaluations using 4 seeds, with the highest scores highlighted in \textbf{bold}.}
% \vspace{-7pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{cc|ccc|cccccc|c}
\toprule

\multirow{2}{*}{\makecell{\textbf{Algo.}}}&\multirow{2}{*}{\textbf{Aug.}}

& \multicolumn{3}{c|}{\textbf{Maze2d}} & \multicolumn{6}{c|}{\textbf{AntMaze}} & \multirow{2}{*}{\textbf{Average}} \\
% \cmidrule{3-11}
&& umaze & medium & large & umaze & medium-play & large-play & umaze-diverse & medium-diverse & large-diverse & \\

\cmidrule{1-12}

& None & 37.41 \footnotesize{$\pm$ 2.83}  & 32.8 \footnotesize{$\pm$ 1.49}  & 58.99 \footnotesize{$\pm$ 9.16}  & 58.75 \footnotesize{$\pm$ 8.9}  & 50.38 \footnotesize{$\pm$ 17.39}  & 78.13 \footnotesize{$\pm$ 3.44}  & 65.5 \footnotesize{$\pm$ 9.46}  & 47.38 \footnotesize{$\pm$ 8.75}  & 45.75 \footnotesize{$\pm$ 6.34}  & 52.79 \footnotesize{$\pm$ 3.46}     \\

&S4RL & 37.69 \footnotesize{$\pm$ 3.36}  & 34.82 \footnotesize{$\pm$ 3.16}  & 62.93 \footnotesize{$\pm$ 3.47}  & 55.0 \footnotesize{$\pm$ 10.47}  & \textbf{51.63 \footnotesize{$\pm$ 11.67} } & \textbf{80.88 \footnotesize{$\pm$ 5.17} } & \textbf{74.0 \footnotesize{$\pm$ 9.72} } & 47.25 \footnotesize{$\pm$ 8.71}  & \textbf{46.13 \footnotesize{$\pm$ 8.34} } & 54.48 \footnotesize{$\pm$ 2.00}   \\

&SynthER & 39.0 \footnotesize{$\pm$ 2.26}  & 34.27 \footnotesize{$\pm$ 2.51}  & 61.74 \footnotesize{$\pm$ 4.51}  & 17.13 \footnotesize{$\pm$ 6.45}  & 23.94 \footnotesize{$\pm$ 11.83}  & 41.0 \footnotesize{$\pm$ 20.58}  & 40.88 \footnotesize{$\pm$ 14.15}  & \textbf{52.38 \footnotesize{$\pm$ 6.48} } & 37.5 \footnotesize{$\pm$ 8.37}  & 38.65 \footnotesize{$\pm$ 3.34}     \\

\rowcolor{Gray}\cellcolor{White}\multirow{-4}{*}{IQL} &GTA  & \textbf{41.68 \footnotesize{$\pm$ 0.0} } & \textbf{37.78 \footnotesize{$\pm$ 0.0} } & \textbf{76.56 \footnotesize{$\pm$ 0.0} } & \textbf{69.75 \footnotesize{$\pm$ 0.0} } & 0.0 \footnotesize{$\pm$ 0.0}  & 79.75 \footnotesize{$\pm$ 0.0}  & 0.0 \footnotesize{$\pm$ 0.0}  & 44.75 \footnotesize{$\pm$ 0.0}  & 0.0 \footnotesize{$\pm$ 0.0}  & \textbf{64.75 \footnotesize{$\pm$ 0.0} }
\\



\bottomrule
\end{tabular}}
\vspace{-0pt}
\label{table:mazes}
\end{table*}



==> tables/novelty_main.tex <==
\begin{table*}
\centering
\caption{
Data quality metrics on D4RL Gym locomotion tasks.}
% \vspace{-7pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{cc|ccc|ccc|ccc|c}
\toprule
\multirow{2}{*}{\makecell{\textbf{Algo.}}} &\multirow{2}{*}{\textbf{Aug.}}

& \multicolumn{3}{c|}{\textbf{Halfcheetah}} & \multicolumn{3}{c|}{\textbf{Hopper}}  & \multicolumn{3}{c|}{\textbf{Walker2d}}& \multirow{2}{*}{\textbf{Average}} \\
% \cmidrule{3-11}
&& medium & medium-replay & medium-expert & medium & medium-replay & medium-expert & medium & medium-replay & medium-expert \\

\cmidrule{1-12}

& None & 48.42 \footnotesize{$\pm$ 0.62}  & 44.64 \footnotesize{$\pm$ 0.71}  & 89.48 \footnotesize{$\pm$ 5.50}  & 61.04 \footnotesize{$\pm$ 3.18}  & 65.69 \footnotesize{$\pm$ 24.41}  & 104.08 \footnotesize{$\pm$ 5.81}  & 84.58 \footnotesize{$\pm$ 1.92}  & 84.11 \footnotesize{$\pm$ 4.12}  & 110.23 \footnotesize{$\pm$ 0.37}  & 76.92 \footnotesize{$\pm$ 2.66}  \\

&S4RL & 48.74 \footnotesize{$\pm$ 0.31}  & 44.53 \footnotesize{$\pm$ 0.30}  & 90.78 \footnotesize{$\pm$ 4.65}  & 59.34 \footnotesize{$\pm$ 3.50}  & 67.39 \footnotesize{$\pm$ 23.81}  & 106.10 \footnotesize{$\pm$ 7.24}  & 84.63 \footnotesize{$\pm$ 2.44}  & 83.42 \footnotesize{$\pm$ 4.70}  & 110.21 \footnotesize{$\pm$ 0.35}  & 77.24 \footnotesize{$\pm$ 3.00}  \\

&SynthER & 49.16 \footnotesize{$\pm$ 0.39}  & 45.57 \footnotesize{$\pm$ 0.34}  & 85.47 \footnotesize{$\pm$ 11.35}  & \textbf{63.70 \footnotesize{$\pm$ 3.69} } & 78.81 \footnotesize{$\pm$ 15.80}  & 98.99 \footnotesize{$\pm$ 11.27}  & 85.43 \footnotesize{$\pm$ 1.14}  & 90.67 \footnotesize{$\pm$ 1.56}  & 109.95 \footnotesize{$\pm$ 0.32}  & 78.64 \footnotesize{$\pm$ 2.38}    \\

\rowcolor{Gray}\cellcolor{White}\multirow{-4}{*}{DynamicMSE} &GTA & \textbf{57.84 \footnotesize{$\pm$ 0.51} } & \textbf{50.04 \footnotesize{$\pm$ 0.84} } & \textbf{93.13 \footnotesize{$\pm$ 3.07} } & 60.89 \footnotesize{$\pm$ 2.91}  & \textbf{89.31 \footnotesize{$\pm$ 16.84} } & \textbf{110.40 \footnotesize{$\pm$ 4.04} } & \textbf{86.69 \footnotesize{$\pm$ 0.89} } & \textbf{93.82 \footnotesize{$\pm$ 1.74} } & \textbf{110.86 \footnotesize{$\pm$ 0.34} } & \textbf{83.66 \footnotesize{$\pm$ 2.04} }
\\

\midrule

 &None & 48.65 \footnotesize{$\pm$ 0.19}  & 43.35 \footnotesize{$\pm$ 0.50}  & 94.57 \footnotesize{$\pm$ 1.88}  & 66.35 \footnotesize{$\pm$ 7.09}  & 95.76 \footnotesize{$\pm$ 4.01}  & 91.69 \footnotesize{$\pm$ 25.97}  & 84.34 \footnotesize{$\pm$ 3.31}  & 69.60 \footnotesize{$\pm$ 10.80}  & 112.37 \footnotesize{$\pm$ 0.60}  & 78.52 \footnotesize{$\pm$ 3.52}  \\

&S4RL & 48.58 \footnotesize{$\pm$ 0.29}  & 43.57 \footnotesize{$\pm$ 0.65}  & 94.22 \footnotesize{$\pm$ 1.59}  & 65.06 \footnotesize{$\pm$ 5.94}  & 86.72 \footnotesize{$\pm$ 22.01}  & 99.82 \footnotesize{$\pm$ 8.09}  & \textbf{84.58 \footnotesize{$\pm$ 4.26} } & 70.33 \footnotesize{$\pm$ 7.99}  & 112.29 \footnotesize{$\pm$ 0.79}  & 78.35 \footnotesize{$\pm$ 2.25}  \\

&SynthER &49.76 \footnotesize{$\pm$ 0.27}  & \textbf{46.91 \footnotesize{$\pm$ 0.28} } & 91.90 \footnotesize{$\pm$ 3.75}  & 69.21 \footnotesize{$\pm$ 5.85}  & \textbf{102.97 \footnotesize{$\pm$ 1.65} } & 94.08 \footnotesize{$\pm$ 23.94}  & 80.15 \footnotesize{$\pm$ 16.47}  & 90.63 \footnotesize{$\pm$ 4.66}  & 112.12 \footnotesize{$\pm$ 0.53}  & 81.97 \footnotesize{$\pm$ 2.21}  \\

\rowcolor{Gray}\cellcolor{White}\multirow{-4}{*}{Oracle reward}& GTA & \textbf{54.82 \footnotesize{$\pm$ 0.35} } & 46.89 \footnotesize{$\pm$ 3.00}  & \textbf{95.30 \footnotesize{$\pm$ 0.55} } & \textbf{72.14 \footnotesize{$\pm$ 3.78} } & 102.11 \footnotesize{$\pm$ 1.51}  & \textbf{107.78 \footnotesize{$\pm$ 4.66} } & 84.40 \footnotesize{$\pm$ 2.32}  & \textbf{93.37 \footnotesize{$\pm$ 6.35} } & \textbf{112.87 \footnotesize{$\pm$ 0.66} } & \textbf{85.52 \footnotesize{$\pm$ 0.90} }
\\
\midrule

&None & 60.98 \footnotesize{$\pm$ 0.72}  & 54.09 \footnotesize{$\pm$ 0.96}  & \textbf{80.51 \footnotesize{$\pm$ 9.45} } & 76.85 \footnotesize{$\pm$ 8.84}  & 101.86 \footnotesize{$\pm$ 0.84}  & 92.85 \footnotesize{$\pm$ 17.35}  & 89.70 \footnotesize{$\pm$ 2.66}  & 92.19 \footnotesize{$\pm$ 1.89}  & \textbf{114.55 \footnotesize{$\pm$ 2.10} } & 84.84 \footnotesize{$\pm$ 1.84}   \\

&S4RL & 60.93 \footnotesize{$\pm$ 0.88}  & 53.32 \footnotesize{$\pm$ 0.99}  & 79.02 \footnotesize{$\pm$ 16.25}  & 73.95 \footnotesize{$\pm$ 10.68}  & 100.62 \footnotesize{$\pm$ 1.84}  & 83.91 \footnotesize{$\pm$ 30.39}  & 90.91 \footnotesize{$\pm$ 0.82}  & 89.90 \footnotesize{$\pm$ 5.44}  & 102.62 \footnotesize{$\pm$ 33.46}  & 81.69 \footnotesize{$\pm$ 3.99}   \\

&SynthER & 63.57 \footnotesize{$\pm$ 0.69}  & \textbf{58.34 \footnotesize{$\pm$ 1.03} } & 45.64 \footnotesize{$\pm$ 7.56}  & 65.61 \footnotesize{$\pm$ 21.89}  & \textbf{103.54 \footnotesize{$\pm$ 0.83} } & \textbf{106.02 \footnotesize{$\pm$ 7.71} } & \textbf{92.31 \footnotesize{$\pm$ 1.04} } & 98.02 \footnotesize{$\pm$ 3.51}  & 112.22 \footnotesize{$\pm$ 1.08}  & 82.81 \footnotesize{$\pm$ 3.21}  \\

\rowcolor{Gray}\cellcolor{White}\multirow{-4}{*}{Novelty}& GTA & \textbf{63.76 \footnotesize{$\pm$ 0.40} } & 54.17 \footnotesize{$\pm$ 2.23}  & 80.00 \footnotesize{$\pm$ 9.03}  & \textbf{77.30 \footnotesize{$\pm$ 8.52} } & 102.19 \footnotesize{$\pm$ 1.09}  & 99.27 \footnotesize{$\pm$ 13.48}  & 91.22 \footnotesize{$\pm$ 3.25}  & \textbf{104.24 \footnotesize{$\pm$ 1.90} } & 111.63 \footnotesize{$\pm$ 1.42}  & \textbf{87.09 \footnotesize{$\pm$ 2.32} }
\\


\bottomrule
\end{tabular}}
\vspace{-0pt}
\label{table:locomotion_main}
\end{table*}



==> tables/robot_and_maze2d.tex <==
\begin{table*}
\centering
\caption{
Normalized average scores on complex robotics tasks like D4RL Adroit, Franka kitchen, and maze2d tasks, with the highest scores highlighted in \textbf{bold}. Each cell displays the mean and standard deviation from 10 evaluations using 4 seeds. All offline RL algorithms trained with dataset augmented by GTA outperform other data augmentation baselines at average scores.}
% \vspace{-7pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{cc|cc|ccc|ccc|c}
\toprule
\multirow{2}{*}{\makecell{\textbf{Algo.}}} &\multirow{2}{*}{\textbf{Aug.}}

& \multicolumn{2}{c|}{\textbf{Adroit}} & \multicolumn{3}{c|}{\textbf{Franka kitchen}}  & \multicolumn{3}{c|}{\textbf{Maze2d}}& \multirow{2}{*}{\textbf{Average}} \\
% \cmidrule{3-11}
&& pen-human & door-human & mixed & partial & complete & umaze & medium & large \\

\cmidrule{1-11}

& None & 44.64 \footnotesize{$\pm$ 0.71}  & 89.48 \footnotesize{$\pm$ 5.50}  & 61.04 \footnotesize{$\pm$ 3.18}  & 65.69 \footnotesize{$\pm$ 24.41}  & 104.08 \footnotesize{$\pm$ 5.81}  & 84.58 \footnotesize{$\pm$ 1.92}  & 84.11 \footnotesize{$\pm$ 4.12}  & 110.23 \footnotesize{$\pm$ 0.37}  & 76.92 \footnotesize{$\pm$ 2.66}  \\

&S4RL & 44.53 \footnotesize{$\pm$ 0.30}  & 90.78 \footnotesize{$\pm$ 4.65}  & 59.34 \footnotesize{$\pm$ 3.50}  & 67.39 \footnotesize{$\pm$ 23.81}  & 106.10 \footnotesize{$\pm$ 7.24}  & 84.63 \footnotesize{$\pm$ 2.44}  & 83.42 \footnotesize{$\pm$ 4.70}  & 110.21 \footnotesize{$\pm$ 0.35}  & 77.24 \footnotesize{$\pm$ 3.00}  \\

&SynthER & 45.57 \footnotesize{$\pm$ 0.34}  & 85.47 \footnotesize{$\pm$ 11.35}  & \textbf{63.70 \footnotesize{$\pm$ 3.69} } & 78.81 \footnotesize{$\pm$ 15.80}  & 98.99 \footnotesize{$\pm$ 11.27}  & 85.43 \footnotesize{$\pm$ 1.14}  & 90.67 \footnotesize{$\pm$ 1.56}  & 109.95 \footnotesize{$\pm$ 0.32}  & 78.64 \footnotesize{$\pm$ 2.38}    \\

\rowcolor{Gray}\cellcolor{White}\multirow{-4}{*}{IQL} &GTA  & \textbf{50.04 \footnotesize{$\pm$ 0.84} } & \textbf{93.13 \footnotesize{$\pm$ 3.07} } & 60.89 \footnotesize{$\pm$ 2.91}  & \textbf{89.31 \footnotesize{$\pm$ 16.84} } & \textbf{110.40 \footnotesize{$\pm$ 4.04} } & \textbf{86.69 \footnotesize{$\pm$ 0.89} } & \textbf{93.82 \footnotesize{$\pm$ 1.74} } & \textbf{110.86 \footnotesize{$\pm$ 0.34} } & \textbf{83.66 \footnotesize{$\pm$ 2.04} }
\\



\bottomrule
\end{tabular}}
\vspace{-0pt}
\label{table:complex_robotics}
\end{table*}



==> tables/temp.tex <==
\begin{table*}
\centering
\caption{Performance of all methods}
% \vspace{7pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{cccc|ccc|ccc|ccc}
\toprule
\multirow{4}{*}{\textbf{Environment}} & \multicolumn{12}{c}{\textbf{D4RL normalized score}}\\ 
\cmidrule{2-13}

& \multicolumn{3}{c|}{\textbf{TD3BC}} & \multicolumn{3}{c|}{\textbf{CQL}}  & \multicolumn{3}{c|}{\textbf{IQL}} & \multicolumn{3}{c}{\textbf{MCQ}} \\
\cmidrule{2-13}
& None & SER & GTA & None & SER & GTA & None  & SER & GTA & None & SER & GTA \\

\cmidrule{1-13}


halfcheetah-m & 48.65 \footnotesize{$\pm$ 0.31} & 49.17 \footnotesize{$\pm$ 0.23} & 57.41 \footnotesize{$\pm$ 0.29} & 46.98 \footnotesize{$\pm$ 0.53} & 47.18 \footnotesize{$\pm$ 0.24} & 53.5 \footnotesize{$\pm$ 0.27} & 48.73 \footnotesize{$\pm$ 0.12} & 49.62 \footnotesize{$\pm$ 0.59} & 55.08 \footnotesize{$\pm$ 0.1} & 61.09 \footnotesize{$\pm$ 0.31} & 63.37 \footnotesize{$\pm$ 0.28} & 63.91 \footnotesize{$\pm$ 0.9} \\
halfcheetah-m-r & 44.77 \footnotesize{$\pm$ 0.7} & 45.53 \footnotesize{$\pm$ 0.33} & 45.72 \footnotesize{$\pm$ 0.44} & 44.37 \footnotesize{$\pm$ 4.9} & 46.07 \footnotesize{$\pm$ 0.25} & 50.62 \footnotesize{$\pm$ 0.36} & 43.5 \footnotesize{$\pm$ 0.53} & 46.86 \footnotesize{$\pm$ 0.35} & 47.34 \footnotesize{$\pm$ 0.46} & 54.23 \footnotesize{$\pm$ 0.31} & 58.31 \footnotesize{$\pm$ 0.41} & 55.31 \footnotesize{$\pm$ 2.55}  \\
halfcheetah-m-e & 92.82 \footnotesize{$\pm$ 2.48} & 82.41 \footnotesize{$\pm$ 6.41} & 63.63 \footnotesize{$\pm$ 15.07} & 95.81 \footnotesize{$\pm$ 10.97} & 94.17 \footnotesize{$\pm$ 0.77} & 93.59 \footnotesize{$\pm$ 0.35} & 94.09 \footnotesize{$\pm$ 2.12} & 90.35 \footnotesize{$\pm$ 5.08} & 92.46 \footnotesize{$\pm$ 2.71} & 81.97 \footnotesize{$\pm$ 2.02} & 45.73 \footnotesize{$\pm$ 3.32} & 54.93 \footnotesize{$\pm$ 3.67}  \\
hopper-m & 61.89 \footnotesize{$\pm$ 3.38} & 63.09 \footnotesize{$\pm$ 2.75} & 57.45 \footnotesize{$\pm$ 4.68} & 62.4 \footnotesize{$\pm$ 4.54} & 63.62 \footnotesize{$\pm$ 3.69} & 61.38 \footnotesize{$\pm$ 3.39} & 64.75 \footnotesize{$\pm$ 6.66} & 68.68 \footnotesize{$\pm$ 3.42} & 62.81 \footnotesize{$\pm$ 8.09} & 83.42 \footnotesize{$\pm$ 4.67} & 79.87 \footnotesize{$\pm$ 6.44} & 74.34 \footnotesize{$\pm$ 8.14}  \\
hopper-m-r & 69.49 \footnotesize{$\pm$ 21.43} & 84.36 \footnotesize{$\pm$ 21.99} & 90.34 \footnotesize{$\pm$ 14.81} & 74.27 \footnotesize{$\pm$ 18.56} & 86.48 \footnotesize{$\pm$ 17.14} & 100.97 \footnotesize{$\pm$ 8.44} & 95.65 \footnotesize{$\pm$ 18.29} & 102.49 \footnotesize{$\pm$ 0.51} & 100.96 \footnotesize{$\pm$ 4.15} & 102.34 \footnotesize{$\pm$ 29.77} & 104.09 \footnotesize{$\pm$ 2.38} & 102.3 \footnotesize{$\pm$ 0.46}  \\
hopper-m-e & 105.91 \footnotesize{$\pm$ 4.63} & 102.04 \footnotesize{$\pm$ 2.04} & 112.47 \footnotesize{$\pm$ 12.02} & 106.08 \footnotesize{$\pm$ 0.23} & 106.95 \footnotesize{$\pm$ 8.01} & 112.07 \footnotesize{$\pm$ 0.55} & 102.02 \footnotesize{$\pm$ 9.74} & 103.13 \footnotesize{$\pm$ 0.26} & 110.45 \footnotesize{$\pm$ 10.59} & 86.85 \footnotesize{$\pm$ 4.46} & 110.63 \footnotesize{$\pm$ 7.63} & 91.9 \footnotesize{$\pm$ 2.19}  \\
walker2d-m & 85.05 \footnotesize{$\pm$ 1.03} & 85.37 \footnotesize{$\pm$ 0.18} & 88.26 \footnotesize{$\pm$ 1.23} & 82.56 \footnotesize{$\pm$ 0.8} & 81.75 \footnotesize{$\pm$ 0.58} & 80.31 \footnotesize{$\pm$ 3.04} & 81.56 \footnotesize{$\pm$ 1.31} & 85.33 \footnotesize{$\pm$ 5.36} & 80.69 \footnotesize{$\pm$ 2.2} & 90.74 \footnotesize{$\pm$ 4.59} & 92.72 \footnotesize{$\pm$ 3.87} & 63.55 \footnotesize{$\pm$ 6.14}  \\
walker2d-m-r & 85.88 \footnotesize{$\pm$ 2.89} & 91.52 \footnotesize{$\pm$ 3.51} & 87.29 \footnotesize{$\pm$ 1.23} & 79.06 \footnotesize{$\pm$ 5.23} & 86.84 \footnotesize{$\pm$ 6.47} & 90.54 \footnotesize{$\pm$ 8.5} & 71.93 \footnotesize{$\pm$ 2.47} & 88.38 \footnotesize{$\pm$ 1.59} & 90.74 \footnotesize{$\pm$ 13.13} & 91.38 \footnotesize{$\pm$ 7.38} & 98.75 \footnotesize{$\pm$ 5.04} & 102.19 \footnotesize{$\pm$ 6.62}  \\
walker2d-m-e & 110.14 \footnotesize{$\pm$ 0.46} & 110.02 \footnotesize{$\pm$ 0.4} & 110.88 \footnotesize{$\pm$ 0.42} & 109.53 \footnotesize{$\pm$ 0.22} & 109.41 \footnotesize{$\pm$ 0.27} & 110.27 \footnotesize{$\pm$ 0.07} & 112.6 \footnotesize{$\pm$ 0.33} & 111.93 \footnotesize{$\pm$ 0.26} & 112.89 \footnotesize{$\pm$ 0.58} & 114.74 \footnotesize{$\pm$ 0.23} & 111.78 \footnotesize{$\pm$ 0.22} & 112.3 \footnotesize{$\pm$ 0.89}  \\







% & PPO & 59.90 & 156.86 & 294.08 & 380.60 & 300.78 & 934.20 & \\
\midrule
\midrule
%\rowcolor{lightgray}
\multirow{1}{*}{Average} &

78.29 \footnotesize{$\pm$ 4.15} & 79.28 \footnotesize{$\pm$ 4.2} & 79.27 \footnotesize{$\pm$ 5.58} & 77.9 \footnotesize{$\pm$ 5.11} & 80.27 \footnotesize{$\pm$ 4.16} & 83.69 \footnotesize{$\pm$ 2.77} & 79.43 \footnotesize{$\pm$ 4.62} & 82.97 \footnotesize{$\pm$ 1.94} & 83.71 \footnotesize{$\pm$ 4.67} & 85.2 \footnotesize{$\pm$ 5.97} & 85.03 \footnotesize{$\pm$ 3.29} & 80.08 \footnotesize{$\pm$ 3.51} \\


\bottomrule
\end{tabular}
}
\label{table:exp_comb}
\end{table*}


